SimCSE: Simple Contrastive Learning of Sentence Embeddings

This paper presents SimCSE, a simple contrastive learning framework that greatly advances state-of-the-art sentence embeddings. We first describe an unsupervised approach, which takes an input sentence and predicts itself in a contrastive objective, with only standard dropout used as noise. This simple method works surprisingly well, performing on par with previous supervised counterparts. We find that dropout acts as minimal data augmentation, and removing it leads to a representation collapse. Then, we propose a supervised approach, which incorporates annotated pairs from natural language inference datasets into our contrastive learning framework by using "entailment" pairs as positives and "contradiction" pairs as hard negatives. We evaluate SimCSE on standard semantic textual similarity (STS) tasks, and our unsupervised and supervised models using BERT base achieve an average of 76.3% and 81.6% Spearman's correlation respectively, a 4.2% and 2.2% improvement compared to the previous best results. We also show -- both theoretically and empirically -- that the contrastive learning objective regularizes pre-trained embeddings' anisotropic space to be more uniform, and it better aligns positive pairs when supervised signals are available.

==> sections/discussion.tex <==
%!TEX root = ../emnlp2021.tex

\section{Discussion}
\label{sec:discussion}

==> sections/method.tex <==
%!TEX root = ../emnlp2021.tex

\section{Background of Contrastive Learning}
\label{sec:contra}

\section{SimCSE}
\label{sec:method}



%In this work, we focus on training a sentence encoder that embeds sentences to real valued dense vectors. These sentence embeddings are expected to be semantically meaningful and can be directly utilized through simple interactions such as cosine similarity.
%To achieve this goal, we formulate the training of the sentence encoder as a contrastive learning problem, where semantically similar sentences are forced be closer in embedding space than dissimilar ones.

In this section, we introduce the framework for contrastive learning, and how we fit our goal of training sentence embeddings into it.

Contrastive learning aims to learn good representation by pulling semantically close neighbors together and pushing apart non-neighbors~\cite{hadsell2006dimensionality}. In our sentence embedding case,
let $\mathcal{D} = \{\langle s_i, s^{+}_i, s^{-}_{i,1},s^{-}_{i,2},\dots,s^{-}_{i,n}\rangle \}_{i=1}^m$ be the training set with $m$ instances, where each instance contains one anchor sentence $s_i$, one positive sentence $s_i^+$ that is semantically similar to $s_i$ and $n$ negative sentences $s^-_{i,j}$ that are semantically dissimilar to the anchor.
For each training step, we randomly sample $N$ instances as a mini-batch,
and we minimize the following objective~\cite{chen2020simple} for each instance in the mini-batch:
% \begin{equation}
% \label{eq:objective}
% \begin{aligned}
%     &\frac{1}{m}\sum_{i=1}^m\mathcal{L}(s_i, s^{+}_i, \{s^{-}_{i,1},s^{-}_{i,2},\dots,s^{-}_{i,n}\}) \\
%     = & - \frac{1}{m}\sum_{i=1}^m\log \frac{e^{\mr{sim}(s_i, s^+_i) / \tau }}{e^{\mr{sim}(s_i, s^+_i) /\tau} + \sum_{j=1}^n e^{\mr{sim}(s_i, s^-_{i,j})/\tau}}
% \end{aligned}
% \end{equation}
\begin{equation}
\label{eq:objective}
\resizebox{.85\hsize}{!}{%
$
\begin{aligned}
    \ell_i = - \log \frac{\exp(\mr{sim}(\mf{h}_i, \mf{h}^+_i) / \tau )}{\sum_{\mf{h}\in \{\mf{h}_i^+,\mf{h}_{i,j}^-\}}\exp(\mr{sim}(\mf{h}_i, \mf{h}) /\tau)},
\end{aligned}
$
}
\end{equation}
where $\mf{h}_i,\mf{h}_i^+,\mf{h}_{i,j}^-$ are encoded  representations corresponding to $s_i,s_i^+,s_{i,j}^-$, $\tau$ is a temperature hyperparameter and $\mr{sim}(\cdot,\cdot)$ is the similarity metric between two embeddings.
% By default, we use pretrained language models such as BERT or RoBERTa to initialize the sentence encoder $E(\cdot)$, and use cosine similarity as similarity metric:
We use the cosine similarity as the metric in both training and the semantic textual similarity tasks:
% \begin{equation}
%     \mr{sim}(s_1, s_2) = \frac{E(s_1)^\mr{T} E(s_2)}{\Vert E(s_1)\Vert_2 \cdot \Vert E(s_2)\Vert_2}
% \end{equation}
\begin{equation}
    \label{eq:similarity}
    \mr{sim}(\mf{h}_1, \mf{h}_2) = \frac{\mf{h}_1^\mr{T} \mf{h}_2}{\Vert \mf{h}_1\Vert_2 \cdot \Vert \mf{h}_2\Vert_2}.
\end{equation}


%In practice, during each training step, we sample a mini-batch of training instances to approximate equation (\ref{eq:objective}).

For getting the sentence representation $\mf{h}$, we encode the input sequence by a pre-trained language model $E$---here we use either BERT~\cite{devlin-etal-2019-bert} or RoBERTa~\cite{liu2019roberta}---and take the \cls~representation as sentence embedding.
% (denoted as \emph{cls}) or take the average hidden representation at each position at both the last layer and the first layer~\cite{li-etal-2020-sentence,su2021whitening}, denoted as \emph{avg}.

% In the following part, we discuss how to construct the contrastive training instances with either unsupervised text or supervised datasets.

% \paragraph{Unsupervised case}

\subsection{Unsupervised SimCSE}

For each anchor sentence in an unsupervised corpus, we simply take itself as its positive sentence, i.e., $s_i=s_i^+$.
For negative sentences, we take the in-batch negative policy~\cite{chen2017sampling,henderson2017efficient}: all other sentences in the same batch serve as the negative samples for this anchor sentence, as shown in Figure~\ref{fig:structure}. Denote $S_i^-$ as the set of negative instances to $s_i$, then in a mini-batch of $N$ instances, each anchor has $|S_i^-|=N-1$.
%gillick2019learning, karpukhin-etal-2020-dense}

The critical flavouring in unsupervised SimCSE to avoid collapsing is \textit{dropout augmentation}. Denote $h^z=E(s, z)$ as encoding sentence $s$ with a random noise $z$ for dropout, we optimize the following objective for the $i$-th sentence in the batch,

\begin{equation}
    \label{eq:unsup_objective}
    \begin{aligned}
        \ell_i = - \log \frac{\exp(\mr{sim}(\mf{h}_i^z, \mf{h}_i^{z'}) / \tau )}{\sum_{j=1}^N\exp(\mr{sim}(\mf{h}_i^z, \mf{h}_j^{z'}) /\tau)}.
    \end{aligned}
\end{equation}

\input{tables/identical_main.tex}
\input{tables/identical_data_aug.tex}
\input{tables/identical_drop.tex}

We view it as a special form of data augmentation: the model takes embeddings of the same sentence---but with different dropouts---as positive pairs.
One may connect our approach to those contrastive learning methods taking neighboring sentences as positive pairs~\cite{logeswaran2018an-quick-thought}, or those augmenting one sentences with different views~\cite{wu2020clear,meng2021coco}.
To compare them, we sample 1 million sentences from Wikipedia (for we find that more data does not significantly help), and train both shared encoders and dual encoders---using distinct models to encode anchor sentences and candidates~\cite{logeswaran2018an-quick-thought}---over these different pairs.
Table~\ref{tab:sts_dataset_identical} shows that, surprisingly, \ours largely outperforms all other variants. We further investigate different data augmentations in Table~\ref{tab:data_aug} and show that even a minimal augmentation (randomly deleting one word) leads to significant drop from using the same sentence.
We also try different dropout rates for the encoders (Table~\ref{tab:drop}) and find out that the default 0.1 dropout rate of transformers~\cite{vaswani2017attention} works the best.
\todo{Show that without dropout the model collapsed.}



% We name this as \textit{identical} contrastive learning. It is connected to the data-augmentation-based contrastive learning in computer vision~\cite{chen2020simple,he2020momentum} and natural language processing~\cite{wu2020clear,meng2021coco}, where different views of the same instance are regarded positive pairs. Though unintuitive, we find that in the case of sentence embeddings, identical contrastive learning \textit{without any data augmentation} works, and works better than its counterparts taking data augmentation. Through theoretical analysis and experiments in \S\ref{sec:claim_reg}, we will show that identical contrastive learning is essentially a regularization of the pre-trained embeddings, and considering the inherent difficulty of data augmentation in NLP, taking extra effort in it may actually backfire.


% \subsection{Unsupervised contrastive learning}
% In our unsupervised setting, the training process is free of human labels and data augmentation techniques. We take the anchor sentence itself as the positive instance, and use in-batch negatives \cite{henderson2017efficient, gillick2019learning, karpukhin-etal-2020-dense} to obtain dissimilar sentences. By this simple approach, unlabeled data without any additional transformation can be utilized for contrastive learning.
%
% Specifically, during each training step we will sample $N$ sentences $\{s_1, s_2, \dots, s_N\}\subseteq \mc{S}$ as a mini-batch, where $\mc{S}$ denotes the training set with unlabeled sentences. Let $\mf{h}_i = \frac{E(s_i)}{\Vert E(s_i) \Vert_2}$, the objective in equation (\ref{eq:objective}) can be rewritten as:
% \begin{equation}
% \label{eq:identical_obj}
% \begin{aligned}
% &\frac{1}{N}\sum_{i=1}^N \mc{L}(s_i, s_i, \{s_j\}_{1 \leq j\leq N, j \ne i}) \\
% =& -\frac{1}{N} \sum_{i=1}^N \log \frac{e^{\mf{h}_i^\mr{T} \mf{h}_i / \tau}}{\sum_{j=1}^N e^{\mf{h}_i^\mr{T} \mf{h}_j / \tau}} \\
% =& - \frac{1}{\tau} + \frac{1}{N}\sum_{i=1}^N \log \sum_{j=1}^N e^{\mf{h}^\mr{T}_i \mf{h}_j / \tau}
% \end{aligned}
% \end{equation}
%We name this way of unsupervised contrastive learning as \textit{identical contrastive learning}.

\begin{comment}
\textbf{Discussion}, it's not so intuitive why using identical sentence pairs as positive instances would bring any help. However, following the arguments similar to \citet{gao2018representation}, identical contrastive learning can be interpreted as a regularization to the sentence embeddings produced by pre-trained language models, which can help ease the anisotropy problem \cite{gao2018representation,li-etal-2020-sentence}. Note that when applying Jensen's inequality to equation (\ref{eq:identical_obj}), we have:
\begin{equation}
\begin{aligned}
&\frac{1}{N}\sum_{i=1}^N \mc{L}(s_i, s_i, \{s_j\}_{1 \leq j\leq N, j \ne i}) \\
=& \log N - \frac{1}{\tau} + \frac{1}{N}\sum_{i=1}^N \log \frac{1}{N}\sum_{j=1}^N e^{\mf{h}^\mr{T}_i \mf{h}_j / \tau} \\
\geq& \log N - \frac{1}{\tau} + \frac{1}{\tau N^2} \sum_{i=1}^N \sum_{j=1}^N \mf{h}^\mr{T}_i \mf{h}_j
\end{aligned}
\end{equation}
ignore some constant terms, identical contrastive learning is actually minimizing an upper bound of
\begin{equation}
\label{eq:indentical_upper}
    \frac{1}{N^2}\sum_{i=1}^N \sum_{j=1}^N\mf{h_i}^\mr{T}\mf{h_j}
\end{equation}
Let full-batch $\mc{S} = \{s_1, s_2, \dots, s_m\}$, and let $\mf{W}$ be the sentence embedding matrix when apply $E(\cdot)$ to $\mc{S}$, i.e. the $i$-th row of $\mf{W}$ is $\mf{h_i}$, we can approximate the summation of all elements in $\mf{W}\mf{W}^\mr{T}$ with equation (\ref{eq:indentical_upper}):
\begin{equation}
\begin{aligned}
        \frac{1}{m^2}\mr{Sum}(\mf{W}\mf{W}^\mr{T}) &= \frac{1}{m^2}\sum_{i=1}^m \sum_{j=1}^m \mf{h}_i^\mf{T}\mf{h}_j \\
    &\approx \frac{1}{N^2}\sum_{i=1}^N \sum_{j=1}^N \mf{h}_i^\mf{T}\mf{h}_j
\end{aligned}
\end{equation}
By classical linear algebra \cite{MERIKOSKI1984177}, $\mr{Sum}(\mf{W}\mf{W}^\mr{T})$ is an upper bound for the singular value of $\mf{W}$ with largest absolute value. Therefore, when taking equation (\ref{eq:identical_obj}) as objective function, we are approximately flattening the singular spectrum of the embedding space.

\end{comment}

%\subsection{Supervised contrastive learning}

\subsection{Supervised SimCSE.}

There are many existing supervised datasets providing sentence pairs that have semantically-close meanings: paraphrasing datasets, NLI datasets, etc. We can utilize these data and take each sentence and its paired one as $s_i$ and $s_i^+$. Again, we take the in-batch negative policy and each anchor sentence has $N-1$ negative samples then.

% \begin{equation}
%     \label{eq:sup_objective}
%     \begin{aligned}
%         \ell_i = - \log \frac{\exp(\mr{sim}(\mf{h}_i, \mf{h}_i^+) / \tau )}{\sum_{j=1}^N\exp(\mr{sim}(\mf{h}_i, \mf{h}_j^+) /\tau)}.
%     \end{aligned}
% \end{equation}

\paragraph{Comparing datasets.}
To figure out what pairwise signal works the best for sentence embeddings with a contrastive objective, we collect a number of datasets with sentence-pair supervision,
%%% paraphrasing
% We take paraphrasing supervised datasets including
% MRPC~\cite{dolan-brockett-2005-automatically-mrpc},
% Language-Net~\cite{lan-etal-2017-continuously-language-net},
% PAWS~\cite{zhang-etal-2019-paws},
% and QQP\footnote{\url{https://www.quora.com/q/quoradata/}}.
namely QQP\footnote{\url{https://www.quora.com/q/quoradata/}}, a question paraphrasing dataset, ParaNMT~\cite{wieting-gimpel-2018-paranmt}, a large-scale back-translation-constructed paraphrasing dataset,
% For these datasets we only take the paraphrasing pairs.
%%% image caption
Flickr30k~\cite{young-etal-2014-image-flickr30k}, an image caption dataset where each image has 5 manually-written captions\footnote{We assume that pairs of captions related to the same image are paraphrasing sentence pairs.}, and natural language inference datasets, including SNLI~\cite{bowman-etal-2015-large-snli} and MNLI~\cite{williams-etal-2018-broad-mnli}.


\input{tables/sts_dataset.tex}


Besides the sizes and corpora, the above datasets differ in several aspects: the paraphrasing or entailment relations are manually verified in QQP and NLI, but not in Flickr30k or ParaNMT. Except NLI where the hypotheses are written by the annotators, all other datasets collect the sentence from existing corpora. We also characterize these pairwise datasets by \emph{lexical overlap}, which is the average F1 score of distinct word sets between sentences in one pair. % (shown in Table~\ref{tab:sts_dataset}).

% We characterize them in three aspects: \emph{lexical overlap} between pairs, whether pairs are \emph{manually verified} to have paraphrasing or entailment relations and whether  pairs are \emph{written by human}. For lexical overlap, we calculate the average F1 score of distinct word sets beatween sentences in one pair. % (shown in Table~\ref{tab:sts_dataset}). The three characteristics are shown in Table~\ref{tab:sts_dataset}.

We train the contrastive model with different datasets and demonstrate in Table~\ref{tab:sts_dataset} that NLI entailment pairs work the best. Considering the dataset characteristics, the result is reasonable:
We expect the training pairs to be of high quality, but also to be challenging to vanilla pre-trained embeddings, which essentially asks for manually verified pairs with low lexical overlap.
While those paraphrasing datasets are collected either using simple retrieval (e.g., TF-IDF) or data augmentation (e.g., back-translation), which lead to high lexical overlap, in NLI, annotators are required to manually write hypotheses as short as possible for a given premise. From another perspective, entailment relation does not require to preserve all information from the premise, thus allows more diverse hypotheses.
All these contribute to high-quality entailment pairs with a low lexical overlap.

% Among all manually-verified datasets, only NLI entailment has a lexical overlap lower than 50\%.


% Table~\ref{tab:sts_dataset} demonstrates the STS performance with different supervised datasets, and the model using NLI entailment data performs far better than others. To eliminate the effects of data sizes, we also downsample each dataset to 134k pairs (the size of QQP) and compare them. The trends are consistent with the original dataset, though the performance of Flickr30k and ParaNMT actually increase with fewer instances. We suspect that since the pairs from the two datasets can be noisy, performance of taking different subsets could vary.

\paragraph{Contradiction as hard negatives.}
We further exploit the nature of NLI data and take the corresponding contradiction hypothesis as hard negative.
In NLI datasets, given one premise, annotators are required to manually write one sentence that is absolutely true (\emph{entailment}), one that is probably true (\emph{neutral}), and one that is definitely false (\emph{contradiction}). Thus for each premise and its entailed hypothesis, there is an accompanying contradicted hypothesis\footnote{In fact, one premise can have multiple contradiction hypotheses in the datasets. In our implementation we only sample one as the hard negative and we did not find that sampling multiple ones would bring a significant difference.}, which looks similar to the premise but expresses opposite meaning. It makes the contradiction hypotheses a perfect source as hard  negatives. Table~\ref{tab:nli_exp} gives an example of a group of NLI instances.

\begin{table}[ht]
    \centering
    \resizebox{0.98\columnwidth}{!}{%
    \begin{tabular}{ll}
        \toprule
        \tf{Premise} & Two dogs are running through a field. \\
        \midrule
        \tf{Entailment} & There are animals outdoors. \\
        \tf{Neutral} & Some puppies are running to catch a stick. \\
        \tf{Contradiction} & The pets are sitting on a couch. \\
        \bottomrule
    \end{tabular}
    }
    \caption{An example of the SNLI dataset from \citet{bowman-etal-2015-large-snli}.}
    \label{tab:nli_exp}
\end{table}

For each anchor sentence $s_i$, denote its entailment and contradiction hypothesis as $s_i^+$ and $s_i^*$, and corresponding embedding as $h_i^+$ and $h_i^*$, we have the following optimization objective,

\todo{Change all sim -> hTh to save space. Mention that h is already normalized.}

\begin{equation}
    \label{eq:sup_objective}
\resizebox{.85\hsize}{!}{%
$
    \begin{aligned}
        \ell_i = - \log \frac{\exp(\mf{h}_i^\mr{T}\mf{h}_i^+ / \tau )}{\sum_{j=1}^N\exp(\mf{h}_i^{\mr{T}}\mf{h}_j^+/\tau)+\exp(\mf{h}_i^{\mr{T}}\mf{h}_j^*/ \tau)}.
    \end{aligned}
$
}
\end{equation}

It is worth noting that  \citet{karpukhin-etal-2020-dense,xiong2021approximate} also incorporate hard negatives by retrieving easy-to-confuse instances with BM25 or dense retriever, which brings significant improvement.

%Specially, we incorporate \emph{contradiction} data as \emph{hard negatives} for NLI datasets.
%This is related to how the two NLI datasets we use --- SNLI~\cite{bowman-etal-2015-large-snli} and MNLI~\cite{williams-etal-2018-broad-mnli} --- are constructed:




% In supervised setting, we assume for each anchor sentence in the training set, there's a labeled positive sentence and a set of labeled negative sentences. Since the amount of labeled negative sentences are usually small, and even zero, we still use in-batch negatives to obtain most of the dissimilar sentences and use labeled negative sentences as hard negatives.

% Specifically, during each training step we will sample $N$ instances $\{\langle s_i, s^+_i, \{s^-_{i,j}\}_{j=1}^n\rangle\}_{i=1}^N \subseteq \mc{S}$. The objective in equation (\ref{eq:objective}) can now be written as:
% \begin{equation}
% \label{eq:supervised_obj}
% \begin{aligned}
% &\frac{1}{N}\sum_{i=1}^N \mc{L}(s_i, s^+_i, \bigcup_{k=1}^N \{s^-_{k,j}\}_{j=1}^n\cup \{s_j\}_{1 \leq j\leq N, j \ne i}) \\
% = &\frac{1}{N}\sum_{i=1}^N\log\frac{e^{\frac{\mf{h}_i^\mr{T}\mf{h}^+_{i}}{\tau}}}{\sum_{j=1}^N e^{\frac{\mf{h}_i^\mr{T}\mf{h}^+_{j}}{\tau}} + \sum_{j=1}^N \sum_{k=1}^n e^{\frac{\mf{h}_i^\mr{T}\mf{h}^-_{j,k}}{\tau}}}
% \end{aligned}
% \end{equation}


% Discrepancies of the datasets


==> tables/batch_size.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table}[t]
    \begin{center}
    \centering
    \resizebox{0.98\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
        \tf{Batch size} & 32 & 64 & 128 & 256 & 512 & 1024\\
    \midrule
        \tf{STS-B} & 84.6 & 85.6 &86.0 &   \tf{86.2} & \tf{86.2} & 86.0 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}

    \caption{
        Effect of different batch sizes (STS-B development set, Spearman's correlation, BERT\ba).
    }
    \vspace{-2pt}
    \label{tab:batch_size}
\end{table}




==> tables/dual_encoder.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table}[ht]
    \begin{center}
    \centering
    \small
    %\resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{lcc}
    \toprule
        \tf{Model} & Shared encoder & Dual encoder\\
    \midrule
    %    \tf{STS-B} & \tf{87.38} & 84.54 \\
        \tf{STS-B} &  \tf{86.18} &84.17 \\
    \bottomrule
    \end{tabular}
    %}
    \end{center}

    \caption{
        Effects of dual encoders.
    }
    \label{tab:dual_encoder}
\end{table}

==> tables/flow_whitening_sts.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table*}[t]
    \begin{center}
    \centering
    \small
    %\resizebox{0.98\textwidth}{!}{%
    
    \begin{tabular}{lcccccccc}
    \toprule
       \tf{Model} & \tf{STS12} & \tf{STS13} & \tf{STS14} & \tf{STS15} & \tf{STS16} & \tf{STS-B} & \tf{SICK-R} & \tf{Avg.} \\
    \midrule
    % \midrule
    %     \multicolumn{9}{c}{\it{Published in \citet{li-etal-2020-sentence} and \citet{su2021whitening}}}\\
    % \midrule
    %     BERT\ba-flow (NLI)$^\spadesuit$ & 59.54 & 64.69 & 64.66 & 72.92 & 71.84 & 58.56 & 65.44 & 65.38\\ 
    %     BERT\ba-flow (target)$^\spadesuit$ & 63.48 & 72.14 & 68.42 & 73.77 & 75.37 & 70.72 & 63.11 & 69.57\\ % target
    %     BERT\ba-whitening (NLI)$^\spadesuit$ & 61.69 & 65.70 & 66.02 & 75.11 & 73.11 & 68.19 & 63.60 & 67.63\\ 
    %     BERT\ba-whitening (target)$^\spadesuit$ & 63.62 & 73.02 & 69.23 & 74.52 & 72.15 & 71.34 & 60.60 & 69.21\\ % target
    %     SBERT\ba-flow (NLI)$^\spadesuit$ & 67.75 & 76.73 & 75.53 & 80.63 & 77.58 & 79.10 & 78.03 & 76.48\\ 
    %     SBERT\ba-flow (target)$^\spadesuit$ & 68.95 & 78.48 & 77.62 & 81.95 & 78.94 & 81.03 & 74.97 & 77.42 \\
    %     SBERT\ba-whitening (NLI)$^\spadesuit$ & 69.11 & 75.79 & 75.76 & 82.31 & 79.61 & 78.66 & 76.33 & 76.80\\ 
    %     SBERT\ba-whitening (target)$^\spadesuit$ & 69.01 & 78.10 & 77.04 & 80.83 & 77.93 & 80.50 & 72.54 & 76.56\\ 
    %     SBERT\la-whitening (target)$^\spadesuit$ & \todon\\
    % \midrule
    \midrule
        \multicolumn{9}{c}{\it{Unsupervised models}}\\
    \midrule
        GloVe embeddings (avg.)$^\clubsuit$ & 55.14 & 70.66 & 59.73 & 68.25 & 63.66 & 58.02 & 53.76 & 61.32 \\
        % FastSent &  \todon \\
        % Quick Thoughts & \todon \\
        % RoBERTa embeddings (\cls) & 16.67&	45.57&	30.36&	55.07&	56.98&	38.81&	61.89&	43.62\\    
        % RoBERTa embeddings (avg.) & 32.10&	56.33&	45.22&	61.35&	61.98&	55.39&	62.03&	53.49\\
        IS-BERT\ba~(NLI)$^\heartsuit$ & 56.77 & 69.24 & 61.21 & 75.23 & 70.16 & 69.21 & 64.25 & 66.58 \\
        CLEAR\ba$^\heartsuit$ & 49.00 & 48.90 & 57.40 & 63.60 & 65.60 & 72.50 & 75.60 & 61.80\\
        BERT\ba & 39.70&	59.38&	49.67&	66.03&	66.19&	53.87&	62.06&	56.70\\ %avg-top-bottom
        BERT\ba-flow (NLI) & 58.40&	67.10&	60.85&	75.16&	71.22&	68.66&	64.47&	66.55 \\
        % \tableindent + flow (target) & 53.15&	78.38&	66.02&	62.09&	70.84&	71.70 &	61.97&	66.31 \\
        BERT\ba-whitening (NLI) & 57.83& 66.90 & 60.90 & 75.08& 71.31& 68.24& 63.73& 66.28\\
        % \tableindent + whitening (target) & 42.88&	77.77&	66.27&	63.60&	67.58&	71.34&	60.40&	64.26\\ % top-bottom
        % \ours-BERT\ba-\identical~(NLI) &62.16&	73.97&	65.40&	74.08&	75.60&	67.68&	66.41&	69.33 \\%62.42&	73.81&	64.91&	74.64&	73.81&	69.73&	67.36&	69.53\\
        \ours-BERT\ba-\identical~(Wiki) & \tf{66.68}&	\tf{81.43} &	\tf{71.38}&	\tf{78.43}&	\tf{78.47}&	\tf{75.49}&	\tf{69.92}&	\tf{74.54}\\
        % jBERT\la & 35.20&	58.78&	48.12&	58.41&	65.90&	54.44&	58.06&	54.13\\
        % jBERT\la-whitening (NLI) & 55.91&	67.66&	61.51&	74.6&	73.7&	68.03&	62.68&66.30 \\
        % jBERT\la-whitening (target) &39.17&	76.72&	65.89&	60.25&	67.51&	71.51&	59.5&62.94\\
        % \midrule 
        % \midrule
        \midrule
        RoBERTa\ba & 40.88&	58.74&	49.07&	65.63&	61.48&	58.55&	61.63&	56.57\\
        % %RoBERT\baa-whitening (cls) & 35.92&	71.94&	60.78&	66.40&	67.18&	68.40&	64.33&	62.14\\
        RoBERTa\ba-whitening (NLI) & 46.99& 63.24&	57.23&	71.36&	68.99&	61.36&	62.91& 61.73\\
        % \tableindent + whitening (target) & 42.54&	77.24&	67.14&	64.25&	67.25&	71.54&	59.62&	64.23\\
        % \ours-RoBERTa\ba-\identical~(NLI) & 63.66&	79.33&	70.26&	79.29&	77.24&	75.01&	64.97&	72.82\\ %63.01&	79.01&	70.64&	78.91&	76.80&	74.45&	65.76&	72.65\\ % cls
        \ours-RoBERTa\ba-\identical~(Wiki) & \tf{68.68}&	\tf{82.62}&	\tf{73.56}&	\tf{81.49}&	\tf{80.82}&	\tf{80.48}&	\tf{67.87}&	\tf{76.50}\\
        % RoBERTa\la & 41.24&	55.82&	47.99&	64.01&	57.81&	53.47&	56.95&	53.90\\
        % RoBERTa\la-whitening (NLI) & 45.89	&63.43&	56.38&	70.64&	68.2&	59.35&	58.65&60.36\\
        % RoBERTa\la-whitening (target) & 41.12&	76.89&	67.41&	66.11&	67.17&	70.65&	56.5&63.69\\
        %BERT-flow (NLI)$^*$ & 59.54 & 64.69 & 64.66 & 72.92 & 71.84 & 58.56 & 65.44 & 65.38\\
        % BERT-whitening-256 (NLI)$^+$ & 61.46 & 66.71 & 66.17 & 74.82 & 72.10 & 67.51 & 64.90 & 67.67\\
        % BERT-whitening-256 (target)$^+$ & 63.89 & 73.76 & 69.08 & 74.59 & 74.40 & 71.43 & 62.20 & 69.91 \\
        % BERT-identical (avg., NLI) & 62.42&	73.81&	64.91&	74.64&	73.81&	69.73&	67.36&	69.53\\
        \midrule
        \ours-BERT\la-\identical~(Wiki) &  67.34&	81.98&	72.36&	81.16&	78.01&	77.10&	74.37&	76.05\\
        \ours-RoBERTa\la-\identical~(Wiki) & 69.87&	82.97&	74.25&	83.01&	79.52&	81.23&	71.47&	77.47 \\
        % RoBERTa-\identical~(avg.) & 63.84&	77.62&	71.57&	78.88&	78.23&	74.78&	66.62&	73.08\\
    \midrule
    \midrule
        \multicolumn{9}{c}{\it{Supervised models}}\\
    \midrule
        InferSent-GloVe$^\clubsuit$ & 52.86 & 66.75 & 62.15 & 72.77 & 66.87 & 68.03 & 65.65 & 65.01\\
        Universal Sentence Encoder$^\clubsuit$ & 64.49 & 67.80 & 64.61 & 76.83 & 73.18 & 74.92 & 76.69 & 71.22 \\
        SBERT\ba~(last avg.)$^\clubsuit$ & 70.97 & 76.53 & 73.19 & 79.09 & 74.30 & 77.03 & 72.91 & 74.89\\
        SBERT\ba~(first-last avg.) &72.57&	74.72&	72.37&	81.72&	75.41&	77.63&	74.84&	75.61\\
        SBERT\ba-flow (NLI) & 69.63&	77.32&	74.14&	81.29&	76.72&	78.15&	76.34&	76.23 \\
        % \tableindent + flow (target) & 66.18&	82.69&	76.22&	73.72&	75.71&	79.99&	73.82&	75.48 \\
        SBERT\ba-whitening (NLI) & 69.61&	75.38&	73.12&	81.91&	77.80&	78.72&	76.35&	76.13 \\
        % \tableindent + whitening (target) & 52.91&	81.91&	75.44&	72.24&	72.93&	80.50&	72.54&	72.64\\
        \ours-BERT\ba & \tf{75.30}&	\tf{84.67}&	\tf{80.19} &	\tf{85.40} &	\tf{80.82} &	\tf{84.25} &	\tf{80.39} &	\tf{81.57} \\
        \midrule
        % \tableindent w/ MLM & 74.9&	80.61&	78.63&	85.17&	80.58&	84.35&	80.34&	80.65 \\
        % SBERT\la$^\clubsuit$ & \todon \\
        % \tableindent + flow  & 74.91&	82.92&	78.75&	85.19&	78.79&	81.47&	75.22&	79.61\\
        % \tableindent + whitening (NLI) & 69.69&	76.19&	73.98&	82.16&	79.35&	79.62&	75.96&	76.71\\
        % \tableindent + whitening (target) & 50.42&	82.23&	75.80 &	73.11&	72.61&	81.1&	71.69&	72.42\\
        SRoBERTa\ba~(last avg.)$^\clubsuit$ & 71.54 & 72.49 & 70.80 & 78.74 & 73.69 & 77.77 & 74.46 & 74.21\\
        SRoBERTa\ba~(first-last avg.) \\
        % SRoBER\baTa & 70.92&	73.03&	70.80&	78.37&	73.68&	77.33&	74.40&	74.08\\
        SRoBERTa\ba-whitening (NLI) & \todon \\
        % \tableindent + whitening (target) & 63.47&	80.27&	69.36&	80.28&	73.93&	80.69&	74.15&	74.59\\
        % SBERT-NLI-flow (target)$^*$ & 68.95 & 78.48 & 77.62 & 81.95 & 78.94 & 81.03 & 74.97 & 77.42 \\
        % SBERT-NLI-whitening-256 (target)$^+$ & 69.97 & 79.48 &  78.12 & 81.60 & 79.07 & 80.80 &  75.06 & 77.73\\
        % SBERT & 70.97&	76.53&	73.19&	79.09&	74.30&	76.98&	72.91&	74.85\\
        % SBERT-NLI-whitening (target, wmean)$^+$ & 69.01 & 78.10 & 77.04 & 80.83 & 77.93 & 80.50 & 72.54 & 76.56\\
        %SBERT-NLI-whitening (target, wmean) & 68.40 & 76.71 & 77.36 & 79.90 & 77.44 & 81.09 & 74.79 & 76.53\\
        % SBERT-NLI-whitening (target, all) & 58.87 & 78.87 & 76.70 & 72.45 & 73.66 & 81.09 & 74.79 & 73.77\\
        %\ours (\cls) & 74.21&	80.01&	74.00&	83.84&	81.01&	82.67&	77.60&	79.05\\
        %\ours-contra (\cls) & 76.56&	82.17&	77.52&	85.75&	82.23&	84.42&	81.01&	81.38\\
        %\ours-contra (avg.) & 72.40&	83.00&	78.05&	85.36&	82.53&	84.96&	80.89&	81.03\\
        %SBERT$_{\texttt{large}}$-NLI-whitening-384 (target)$^+$ & 71.25 & 80.05 & 78.96 & 82.53 & 80.36 & 82.22 & 74.05 & 78.49\\
        %\ours-contra+mlm+penalty & 72.90&	83.95&	78.66&	85.43&	81.80&	85.20&	80.79&	81.25\\
        \ours-RoBERTa\ba & 76.53&	85.21&	80.95&	86.03&	82.57&	85.83&	80.50&	82.52\\ % l=32
        \midrule
        % \tableindent w/ MLM & 75.40&	84.11&	79.47&	85.69&	82.08&	85.87&	80.38&	81.86 \\
        % SRoBERTa\la$^\clubsuit$ & \todon\\
        % % SRoBER\baTa & 70.92&	73.03&	70.80&	78.37&	73.68&	77.33&	74.40&	74.08\\
        % SRoBERTa\la-whitening (NLI) & \todon \\
        % SRoBERTa\la-whitening (target) & \todon \\
        \ours-BERT\la & 75.78&	86.33&	80.44&	86.06&	80.86&	84.87&	81.14&	82.21\\
        \ours-RoBERTa\la & 77.46&	87.27&	82.36&	86.66&	83.93&	86.70&	81.95&	83.76\\
        %SBERT-whitening (target)$^\spadesuit$ & 69.01 & 78.10 & 77.04 & 80.83 & 77.93 & 80.50 & 72.54 & 76.56\\ 
        %\ours-contra-norm (wmean) & 71.57 & 81.41 & 80.23 & 84.14 & 83.15 & 85.83 & 80.50 & 80.98\\
        %\ours$_{\texttt{large}}$-contra-norm & 77.75&	87.08&	81.86&	86.01&	83.60&	86.11&	81.04&	83.35\\
    % \midrule
    %     \multicolumn{9}{c}{Large results}\\
    % \midrule
    %     RoBERTa embeddings (\cls) & 19.23&	22.91&	14.91&	33.39&	38.00&	17.31&	40.67&	26.63\\
    %     RoBERTa embeddings (avg.) & 33.61&	57.23&	45.66&	62.99&	61.18&	50.56&	58.40&	52.80\\
    %     SRoBERTa & 74.07&	77.10&	73.28&	81.63&	76.90&	78.67&	74.12&	76.54 \\
    %     \ours (\cls) \\
    %     \ours-contra (\cls) \\
    %     \ours-contra (avg.) \\
    \bottomrule
    \end{tabular}
    %}
    \end{center}

    \caption{
        Results of various sentence embedding methods on STS tasks (Spearman's correlation). 
        $\clubsuit$: results from \citet{reimers-gurevych-2019-sentence};
        % $\spadesuit$: results from \citet{li-etal-2020-sentence} and \citet{su2021whitening};
        $\heartsuit$: results from \citet{zhang-etal-2020-unsupervised,wu2020clear} correspondingly; 
        all other results are reproduced by ourselves.
        % $^+$: results from \citet{su2021whitening}. 
        %\ours: contrastive learning using NLI entailment data.
        As described in \S\todo{xx}, evaluation protocols of \citet{li-etal-2020-sentence,su2021whitening} are different from ours, so we list their original numbers separately and reproduce the whitening model under the same setting. 
        For pre-trained models, we use the \ttt{base} version for all results in this table. 
        We take the best pooling methods for different model families (\S\todo{xx}): For \identical~and \ours, we take the \cls~representation, otherwise we take the first-last-avg pooling following \citet{li-etal-2020-sentence,su2021whitening}. 
        \tianyu{Note that we use avg-top-bottom for BERT/RoBERTa-whitening.} \xingcheng{For SBERT-whitening, we do whitening on top of the pre-trained models released by \citet{su2021whitening}; for SBERT-flow, we finetune the BERT and Glow model based on the code released by \citet{li-etal-2020-sentence}}
    }
    \label{tab:flow_whitening_sts}
\end{table*}

==> tables/intro.tex <==
  %!TEX root = ../emnlp2021.tex

\begin{table}[t]
    \centering
    \small
    \resizebox{0.9\columnwidth}{!}{%

    \begin{tabular}{ll}
    \toprule
      &  {BERT\ba} \\
    \midrule
        \ti{Unsupervised} \\
        \tableindent\tableindent Avg. embeddings & 56.7 \\
        \tableindent\tableindent CT-BERT ({prev. SoTA}) & 72.1  \\
        \tableindent\tableindent \ours & \tf{76.3}~(+4.2\%) \\
    \midrule
        \ti{Supervised} \\
        \tableindent\tableindent SBERT  & 74.9  \\
        \tableindent\tableindent CT-SBERT ({prev. SoTA}) & 79.4  \\
        \tableindent\tableindent \ours & \tf{81.6}~(+2.2\%)\\
    \bottomrule
    \end{tabular}
   }

    \caption{
        Comparison between \ours and previous state-of-the-art (unsupervised and supervised). The reported numbers are the average of seven STS tasks (Spearman's correlation), see Table~\ref{tab:main_sts} for details. 
        %IS-BERT, SBERT, SBERT-whitening:  \newcite{zhang-etal-2020-unsupervised}, \newcite{reimers-gurevych-2019-sentence} and \citet{su2021whitening}.
        SBERT, CT: \newcite{reimers-gurevych-2019-sentence} and \newcite{carlsson2021semantic}.
    }
    % \vspace{-10pt}
    \label{tab:intro}
\end{table}


==> tables/pearson_sts.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table*}[t]
    \begin{center}
    \centering
    \small
    %\resizebox{0.98\textwidth}{!}{%
    
    \begin{tabular}{lcccccccc}
    \toprule
       \tf{Model} & \tf{STS12} & \tf{STS13} & \tf{STS14} & \tf{STS15} & \tf{STS16} & \tf{STS-B} & \tf{SICK-R} & \tf{Avg.} \\
    \midrule
        BGT$^\heartsuit$ & 68.9 & 62.2 &  75.9 & 79.4 & 79.3 & - & - & - \\
        ParaBART$^\heartsuit$& 68.4 & 71.1 & 76.4 & 80.7 &80.1 & 78.5 & - & - \\
    \midrule
        % Unsup. \ours-BERT\ba & 67.4&	75.2&	75.1&	78.7&	78.3&	76.1&	77.0&	75.4 \\
        \ours-BERT\ba& 70.8&	76.9&	81.5&	81.8&	79.5&	83.3&	85.1&	79.8\\
        % Unsup. \ours-RoBERTa\ba & 68.9&	76.9&	76.9&	79.2&	80.4&	81.5&	76.7&	77.2 \\
        \ours-RoBERTa\ba& 71.5&	78.7&	82.0&	82.8&	81.0&	84.9&	84.8&	80.8\\
    \bottomrule
    \end{tabular}
    %}
    \end{center}

    \caption{
        STS results with ``mean'' setting (Pearson). 
        $\heartsuit$: results from \citet{wieting-etal-2020-bilingual,huang2021disentangling}. 
        Note that ParaBART takes BART~\cite{lewis-etal-2020-bart}, which is a  more powerful pre-trained language model. 
    }
    \label{tab:pearson_sts}
\end{table*}



==> tables/pooling.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table}[ht]
    \begin{center}
    \centering
    \small
    %\resizebox{0.6\columnwidth}{!}{%
    \begin{tabular}{lcc}
    \toprule
        \tf{Pooling} & \tf{STS-B} & \tf{Avg. transfer} \\
    \midrule
        \cls& 86.18 & 81.55\\
        First-last avg. & 86.13 & 81.61 \\
    \bottomrule
    \end{tabular}
    %}
    \end{center}

    \caption{
        Development set results with different pooling methods. 
        We observe no significant difference of the two pooling methods with \ours.  
        %When using \cls, an MLP layer is applied on top of the representation. 
    }
    \label{tab:pooling}
\end{table}

==> tables/sts_whitening.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table*}[t]
    \begin{center}
    \centering
    \resizebox{0.98\textwidth}{!}{%
    
    \begin{tabular}{lcccccccc}
    \toprule
       \tf{Model} & \tf{STS12} & \tf{STS13} & \tf{STS14} & \tf{STS15} & \tf{STS16} & \tf{STS-B} & \tf{SICK-R} & \tf{Avg.} \\
    \midrule
        BERT (top-bottom, all) & 39.70&	59.38&	49.67&	66.03&	66.19&	53.87&	62.06&	56.70\\
        BERT (top-bottom, wmean) & 54.44  &  58.03 &   58.87 &  67.94 &  68.41 &  53.87 &  62.06 &  60.52\\
        BERT (top-bottom)$^+$ & 57.86 & 61.97 & 62.49 & 70.96 & 69.76 & 59.04 & 63.75 & 63.69\\
    \midrule
        BERT-whitening (target, all) & 42.88&	77.77&	66.27&	63.60&	67.58&	71.34&	60.40&	64.26\\
        BERT-whitening (target, wmean) & 63.38 & 73.01 & 69.13 & 74.48 & 72.56 & 71.34 & 60.40 & 69.19\\
        BERT-whitening (target)$^+$ & 63.62 & 73.02 & 69.23 & 74.52 & 72.15 & 71.34 & 60.60 & 69.21\\
    \midrule
        BERT-identical (NLI) & 62.42&	73.81&	64.91&	74.64&	73.81&	69.73&	67.36&	69.53\\
        BERT-identical (NLI, wmean) & 62.71 & 71.18 & 68.57 & 75.20 & 75.42 & 69.73 & 67.36 & 70.02\\
        BERT-identical-whitening (NLI) & 50.05 & 77.23 & 67.11 & 66.20 & 70.05 & 73.66 & 64.32 & 66.95\\
        BERT-identical-whitening (NLI, wmean) & 63.45 & 71.28 & 69.84 & 75.40 & 73.75 & 73.66 & 64.32 & 70.24\\
    \bottomrule
    \end{tabular}
    }
    \end{center}

    \caption{
       STS results. $\dagger$: results from \citet{reimers-gurevych-2019-sentence}. $^*$: results from \citet{li-etal-2020-sentence}. $^+$: results from \citet{su2021whitening}. \ours: contrastive learning using NLI entailment data. \ours-contra: incorporating contradiction data and cross in-batch negatives. We use the \texttt{base} version for all pre-trained models.
    }
    \label{tab:sts_whitening}
\end{table*}
